Predicting Memory Demands of BDD Operations using Maximum Graph Cuts (Extended Paper)

The BDD package Adiar manipulates Binary Decision Diagrams (BDDs) in external memory. This enables handling big BDDs, but the performance suffers when dealing with moderate-sized BDDs. This is mostly due to initializing expensive external memory data structures, even if their contents can fit entirely inside internal memory. The contents of these auxiliary data structures always correspond to a graph cut in an input or output BDD. Specifically, these cuts respect the levels of the BDD. We formalise the shape of these cuts and prove sound upper bounds on their maximum size for each BDD operation. We have implemented these upper bounds within Adiar. With these bounds, it can predict whether a faster internal memory variant of the auxiliary data structures can be used. In practice, this improves Adiar's running time across the board. Specifically for the moderate-sized BDDs, this results in an average reduction of the computation time by 86.1% (median of 89.7%). In some cases, the difference is even 99.9\%. When checking equivalence of hardware circuits from the EPFL Benchmark Suite, for one of the instances the time was decreased by 52 hours.

==> data/ir_knights_tour_closed_0nodes.tex <==
20.4      100.0 % 6
44.3      100.0 % 7
169.9     100.0 % 8
87.0      85.71 % 9
505.2     100.0 % 10
15328.0   87.27 % 11
225449.6  0.00  % 12
3770721.2 0.00  % 13
3087.9    49.46 % 14


==> data/ir_knights_tour_closed_1level.tex <==
20.4      100.0 % 6
44.3      100.0 % 7
169.9     100.0 % 8
87.0      100.0 % 9
505.2     100.0 % 10
15328.0   90.91 % 11
225449.6  64.18 % 12
3770721.2 59.49 % 13
3087.9    100.0 % 14


==> data/ir_knights_tour_closed_2level.tex <==
20.4      100.0 % 6
44.3      100.0 % 7
169.9     100.0 % 8
87.0      100.0 % 9
505.2     100.0 % 10
15328.0   96.36 % 11
225449.6  65.67 % 12
3770721.2 59.49 % 13
3087.9    100.0 % 14


==> data/ir_knights_tour_open_0nodes.tex <==
23.3      100.0 % 5
112.2     100.0 % 6
103.3     100.0 % 7
223.4     70.97 % 8
375.1     53.85 % 9
70646.9   16.33 % 10
389292.3  0.00  % 11
8246870.8 0.00  % 12


==> data/ir_knights_tour_open_1level.tex <==
23.3      100.0 % 5
112.2     100.0 % 6
103.3     100.0 % 7
223.4     100.0 % 8
375.1     97.44 % 9
70646.9   75.51 % 10
389292.3  64.41 % 11
8246870.8 57.75 % 12


==> data/ir_knights_tour_open_2level.tex <==
23.3      100.0 % 5
112.2     100.0 % 6
103.3     100.0 % 7
223.4     100.0 % 8
375.1     100.0 % 9
70646.9   75.51 % 10
389292.3  64.41 % 11
8246870.8 59.15 % 12


==> data/ir_picotrav_0nodes.tex <==
191.5    100.0 % adder     (depth)
123.6    99.95 % sin       (depth)
18.3     100.0 % cavlc     (depth)
8.3      100.0 % ctrl      (depth)
22.3     100.0 % i2c       (depth)
16.7     100.0 % int2float (depth)
81.3     100.0 % priority  (depth)
33.5     100.0 % router    (depth)
177462.8 95.13 % voter     (depth)
222.5    100.0 % adder     (size)
63256.5  71.80 % sin       (size)
6373.5   99.80 % arbiter   (size)
23.5     100.0 % i2c       (size)
5.7      100.0 % int2float (size)
107.6    100.0 % priority  (size)
33.8     100.0 % router    (size)
69544.2  95.65 % voter     (size)


==> data/ir_picotrav_1level.tex <==
191.5    100.0 % adder     (depth)
123.6    99.97 % sin       (depth)
18.3     100.0 % cavlc     (depth)
8.3      100.0 % ctrl      (depth)
22.3     100.0 % i2c       (depth)
16.7     100.0 % int2float (depth)
81.3     100.0 % priority  (depth)
33.5     100.0 % router    (depth)
177462.8 99.02 % voter     (depth)
222.5    100.0 % adder     (size)
63256.5  75.87 % sin       (size)
6373.5   99.95 % arbiter   (size)
23.5     100.0 % i2c       (size)
5.7      100.0 % int2float (size)
107.6    100.0 % priority  (size)
33.8     100.0 % router    (size)
69544.2  99.11 % voter     (size)


==> data/ir_picotrav_2level.tex <==
191.5    100.0 % adder     (depth)
123.6    99.97 % sin       (depth)
18.3     100.0 % cavlc     (depth)
8.3      100.0 % ctrl      (depth)
22.3     100.0 % i2c       (depth)
16.7     100.0 % int2float (depth)
81.3     100.0 % priority  (depth)
33.5     100.0 % router    (depth)
177462.8 99.11 % voter     (depth)
222.5    100.0 % adder     (size)
63256.5  76.33 % sin       (size)
6373.5   99.95 % arbiter   (size)
23.5     100.0 % i2c       (size)
5.7      100.0 % int2float (size)
107.6    100.0 % priority  (size)
33.8     100.0 % router    (size)
69544.2  99.15 % voter     (size)


==> data/ir_queens_bdd_0nodes.tex <==
42.8      100.0 % 4
107.4     100.0 % 5
238.3     100.0 % 6
609.2     91.67 % 7
1527.7    90.48 % 8
4243.2    91.25 % 9
12617.1   90.91 % 10
42629.3   85.00 % 11
163120.4  79.02 % 12
696820.1  69.64 % 13
3266896.2 63.59 % 14
% 16555232.5 58.93 % 15


==> data/ir_queens_bdd_1level.tex <==
42.8      100.0 % 4
107.4     100.0 % 5
238.3     100.0 % 6
609.2     100.0 % 7
1527.7    100.0 % 8
4243.2    93.75 % 9
12617.1   92.93 % 10
42629.3   93.33 % 11
163120.4  93.71 % 12
696820.1  93.45 % 13
3266896.2 88.72 % 14
% 16555232.5 79.91 % 15


==> data/ir_queens_bdd_2level.tex <==
42.8      100.0 % 4
107.4     100.0 % 5
238.3     100.0 % 6
609.2     100.0 % 7
1527.7    100.0 % 8
4243.2    93.75 % 9
12617.1   93.94 % 10
42629.3   93.33 % 11
163120.4  93.71 % 12
696820.1  94.95 % 13
3266896.2 88.72 % 14
% 16555232.5 79.91 % 15


==> data/ir_queens_zdd_0nodes.tex <==
25.9       100.0 % 4
80.3       100.0 % 5
214.0      100.0 % 6
545.6      93.75 % 7
1326.5     90.48 % 8
3213.0     88.75 % 9
7822.3     81.82 % 10
19894.5    70.83 % 11
54826.2    61.54 % 12
170186.1   54.17 % 13
614963.4   53.33 % 14
2585599.4  40.18 % 15
% 12296445.4 34.90 % 16


==> data/ir_queens_zdd_1level.tex <==
25.9       100.0 % 4
80.3       100.0 % 5
214.0      100.0 % 6
545.6      93.75 % 7
1326.5     100.0 % 8
3213.0     93.75 % 9
7822.3     92.93 % 10
19894.5    93.33 % 11
54826.2    93.71 % 12
170186.1   93.45 % 13
614963.4   93.85 % 14
2585599.4  94.20 % 15
% 12296445.4 94.89 % 16


==> data/ir_queens_zdd_2level.tex <==
25.9       100.0 % 4
80.3       100.0 % 5
214.0      100.0 % 6
545.6      100.0 % 7
1326.5     100.0 % 8
3213.0     93.75 % 9
7822.3     92.93 % 10
19894.5    93.33 % 11
54826.2    93.71 % 12
170186.1   93.45 % 13
614963.4   93.85 % 14
2585599.4  94.20 % 15
% 12296445.4 95.17 % 16

==> data/ir_tic_tac_toe_bdd_0nodes.tex <==
485.0       100.0 % 16
2077.6      100.0 % 17
10292.8     100.0 % 18
59283.9     76.32 % 19
332937.3    63.16 % 20
1767478.8   57.89 % 21
8555218.2   57.89 % 22
% 36573231.9  56.58 % 23
% 132606027.4 56.58 % 24

==> data/ir_tic_tac_toe_bdd_1level.tex <==
485.0       100.0 % 16
2077.6      100.0 % 17
10292.8     100.0 % 18
59283.9     100.0 % 19
332937.3    88.16 % 20
1767478.8   68.42 % 21
8555218.2   63.16 % 22
% 36573231.9  61.84 % 23
% 132606027.4 60.53 % 24

==> data/ir_tic_tac_toe_bdd_2level.tex <==
485.0       100.0 % 16
2077.6      100.0 % 17
10292.8     100.0 % 18
59283.9     10000 % 19
332937.3    92.11 % 20
1767478.8   69.74 % 21
8555218.2   63.16 % 22
% 36573231.9  61.84 % 23
% 132606027.4 60.53 % 24

==> data/ir_tic_tac_toe_zdd_0nodes.tex <==
246.8       100.0 % 16
1153.7      100.0 % 17
6138.7      69.74 % 18
39596.8     61.84 % 19
245775.4    52.63 % 20
1408529.2   50.00 % 21
7207145.8   46.05 % 22
% 32002420.4  42.11 % 23
% 118781618.5 40.79 % 24

==> data/ir_tic_tac_toe_zdd_1level.tex <==
246.8       100.0 % 16
1153.7      100.0 % 17
6138.7      100.0 % 18
39596.8     100.0 % 19
245775.4    76.32 % 20
1408529.2   63.16 % 21
7207145.8   60.53 % 22
% 32002420.4  60.53 % 23
% 118781618.5 59.21 % 24

==> data/ir_tic_tac_toe_zdd_2level.tex <==
246.8       100.0 % 16
1153.7      100.0 % 17
6138.7      100.0 % 18
39596.8     100.0 % 19
245775.4    78.95 % 20
1408529.2   64.47 % 21
7207145.8   61.84 % 22
% 32002420.4  60.53 % 23
% 118781618.5 60.53 % 24

==> data/motivation_queens_adiar_v100.tex <==
7  7.486
8  8.149
9  7.835
10 9.419
11 7.297
12 28.510
13 118.887
14 660.127
15 3943.981
16 31017.033
17 265758.859


==> data/motivation_queens_adiar_v120.tex <==
7  0.105
8  0.163
9  0.361
10 0.841
11 3.137
12 14.844
13 82.715
14 502.855
15 3336.591
16 23127.559
17 199730.402


==> data/motivation_queens_buddy.tex <==
7  0.009
8  0.020
9  0.052
10 0.186
11 0.821
12 4.117
13 23.255
14 142.423


==> data/motivation_queens_cudd.tex <==
7  0.002
8  0.009
9  0.040
10 0.526
11 1.593
12 8.967
13 52.881
14 316.093
15 2687.585


==> data/motivation_queens_sylvan.tex <==
7  0.014
8  0.021
9  0.074
10 0.210
11 0.875
12 7.160
13 45.805
14 309.479
15 1836.749


==> data/motivation_tic_tac_toe_adiar_v100.tex <==
16 1.817
17 1.876
18 2.346
19 4.268
20 29.513
21 124.148
22 599.800
23 2815.244
24 12479.837
25 43574.274
26 104621.760
27 234606.020
28 478232.065


==> data/motivation_tic_tac_toe_adiar_v120.tex <==
16 0.186
17 0.279
18 0.655
19 2.539
20 13.879
21 78.334
22 417.011
23 1913.585
24 7257.237
25 23429.195
26 63569.389
27 162223.297
28 315154.457


==> data/motivation_tic_tac_toe_buddy.tex <==
16 0.004
17 0.022
18 0.092
19 0.575
20 4.032
21 23.371
22 128.102
23 667.436


==> data/motivation_tic_tac_toe_cudd.tex <==
16 0.001
17 0.351
18 0.424
19 1.055
20 7.626
21 48.172
22 255.093
23 1257.012
24 5246.023


==> data/motivation_tic_tac_toe_sylvan.tex <==
16 0.012
17 0.032
18 0.136
19 0.787
20 6.973
21 53.607
22 293.725
23 1386.782
24 5244.662
25 17420.893


==> data/ppr_unweighted_knights_tour_0nodes.tex <==
23.3      0.3333 % 5  (open)
112.2     0.1538 % 6  (open)
103.3     0.0870 % 7  (open)
223.4     0.0345 % 8  (open)
375.1     0.0256 % 9  (open)
70646.9   0.0204 % 10 (open)
389292.3  0.0000 % 11 (open)
8246870.8 0.0000 % 12 (open)
20.4      0.2857 % 6  (closed)
44.3      0.1250 % 7  (closed)
169.9     0.0435 % 8  (closed)
87.0      0.0303 % 9  (closed)
505.2     0.0000 % 10 (closed)
15328.0   0.0000 % 11 (closed)
225449.6  0.0000 % 12 (closed)
3770721.2 0.0000 % 13 (closed)
3087.9    0.0000 % 14 (closed)



==> data/ppr_unweighted_knights_tour_1level.tex <==
23.3      7.333 % 5  (open)
112.2     1.846 % 6  (open)
103.3     1.304 % 7  (open)
223.4     0.966 % 8  (open)
375.1     0.769 % 9  (open)
70646.9   0.633 % 10 (open)
389292.3  0.525 % 11 (open)
8246870.8 0.451 % 12 (open)
20.4      2.143 % 6  (closed)
44.3      1.563 % 7  (closed)
169.9     1.130 % 8  (closed)
87.0      0.848 % 9  (closed)
505.2     0.391 % 10 (closed)
15328.0   0.564 % 11 (closed)
225449.6  0.493 % 12 (closed)
3770721.2 0.430 % 13 (closed)
3087.9    0.170 % 14 (closed)



==> data/ppr_unweighted_knights_tour_2level.tex <==
23.3      7.333 % 5  (open)
112.2     2.615 % 6  (open)
103.3     1.913 % 7  (open)
223.4     1.414 % 8  (open)
375.1     1.128 % 9  (open)
70646.9   0.939 % 10 (open)
389292.3  0.780 % 11 (open)
8246870.8 0.662 % 12 (open)
20.4      2.143 % 6  (closed)
44.3      1.938 % 7  (closed)
169.9     1.478 % 8  (closed)
87.0      1.152 % 9  (closed)
505.2     0.522 % 10 (closed)
15328.0   0.800 % 11 (closed)
225449.6  0.687 % 12 (closed)
3770721.2 0.608 % 13 (closed)
3087.9    0.213 % 14 (closed)


==> data/ppr_unweighted_picotrav_0nodes.tex <==
191.5    4.6055  % adder     (depth)
123.6    13.6911 % sin       (depth)
18.3     9.5067  % cavlc     (depth)
8.3      9.4094  % ctrl      (depth)
9.1      5.6796  % dec       (depth)
22.3     9.6956  % i2c       (depth)
16.7     10.4758 % int2float (depth)
81.3     5.5954  % priority  (depth)
33.5     7.9476  % router    (depth)
177462.8 4.8640  % voter     (depth)
222.5    2.8012  % adder     (size)
63256.5  1.4425  % sin       (size)
6373.5   4.3897  % arbiter   (size)
23.5     10.3691 % i2c       (size)
5.7      10.3691 % int2float (size)
107.6    4.7952  % priority  (size)
33.8     8.4520  % router    (size)
69544.2  4.9518  % voter     (size)



==> data/ppr_unweighted_picotrav_1level.tex <==
191.5    28.5995 % adder     (depth)
123.6    34.7261 % sin       (depth)
18.3     26.9225 % cavlc     (depth)
8.3      25.9280 % ctrl      (depth)
9.1      29.1457 % dec       (depth)
22.3     29.9282 % i2c       (depth)
16.7     28.8161 % int2float (depth)
81.3     38.0402 % priority  (depth)
33.5     36.6262 % router    (depth)
177462.8 17.0231 % voter     (depth)
222.5    36.7401 % adder     (size)
63256.5  3.4759  % sin       (size)
6373.5   27.6617 % arbiter   (size)
23.5     30.7394 % i2c       (size)
5.7      12.9237 % int2float (size)
107.6    41.0252 % priority  (size)
33.8     36.4015 % router    (size)
69544.2  17.2100 % voter     (size)


==> data/ppr_unweighted_picotrav_2level.tex <==
191.5    36.6851 % adder     (depth)
123.6    41.5070 % sin       (depth)
18.3     29.6065 % cavlc     (depth)
8.3      27.6998 % ctrl      (depth)
9.1      29.1457 % dec       (depth)
22.3     31.8009 % i2c       (depth)
16.7     31.6081 % int2float (depth)
81.3     38.1006 % priority  (depth)
33.5     38.8667 % router    (depth)
177462.8 18.8498 % voter     (depth)
222.5    48.5860 % adder     (size)
63256.5  4.5307  % sin       (size)
6373.5   35.6749 % arbiter   (size)
23.5     33.0811 % i2c       (size)
5.7      13.8036 % int2float (size)
107.6    41.8652 % priority  (size)
33.8     38.7652 % router    (size)
69544.2  18.9851 % voter     (size)


==> data/ppr_unweighted_queens_bdd_0nodes.tex <==
42.8       2.200  % 4
107.4      1.6250 % 5
238.3      1.2857 % 6
609.2      1.0625 % 7
1527.7     0.8889 % 8
4243.2     0.7500 % 9
12617.1    0.6465 % 10
42629.3    0.5583 % 11
163120.4   0.4825 % 12
696820.1   0.4286 % 13
3266896.2  0.3795 % 14
16555232.5 0.3348 % 15



==> data/ppr_unweighted_queens_bdd_1level.tex <==
42.8       11.867 % 4
107.4      10.042 % 5
238.3      8.657 % 6
609.2      7.583 % 7
1527.7     6.730 % 8
4243.2     6.050 % 9
12617.1    5.495 % 10
42629.3    5.033 % 11
163120.4   4.643 % 12
696820.1   4.310 % 13
3266896.2  4.021 % 14
16555232.5 3.772 % 15


==> data/ppr_unweighted_queens_bdd_2level.tex <==
42.8       13.000 % 4
107.4      10.708 % 5
238.3      9.086 % 6
609.2      7.875 % 7
1527.7     6.952 % 8
4243.2     6.213 % 9
12617.1    5.626 % 10
42629.3    5.133 % 11
163120.4   4.727 % 12
696820.1   4.381 % 13
3266896.2  4.087 % 14
16555232.5 3.826 % 15


==> data/ppr_unweighted_queens_zdd_0nodes.tex <==
25.9       7.933 % 4
80.3       2.9583 % 5
214.0      1.2857 % 6
545.6      0.6458 % 7
1326.5     0.3651 % 8
3213.0     0.2250 % 9
7822.3     0.1515 % 10
19894.5    0.1083 % 11
54826.2    0.0769 % 12
170186.1   0.0595 % 13
614963.4   0.0462 % 14
2585599.4  0.0357 % 15
12296445.4 0.0275 % 16


==> data/ppr_unweighted_queens_zdd_1level.tex <==
25.9       39.333 % 4
80.3       41.833 % 5
214.0      42.971 % 6
545.6      43.458 % 7
1326.5     44.175 % 8
3213.0     44.925 % 9
7822.3     45.717 % 10
19894.5    46.483 % 11
54826.2    47.266 % 12
170186.1   47.935 % 13
614963.4   48.574 % 14
2585599.4  49.179 % 15
12296445.4 49.702 % 16


==> data/ppr_unweighted_queens_zdd_2level.tex <==
25.9       45.267 % 4
80.3       49.125 % 5
214.0      50.829 % 6
545.6      51.333 % 7
1326.5     51.984 % 8
3213.0     52.538 % 9
7822.3     53.101 % 10
19894.5    53.608 % 11
54826.2    54.133 % 12
170186.1   54.560 % 13
614963.4   54.979 % 14
2585599.4  55.388 % 15
12296445.4 55.729 % 16


==> data/ppr_unweighted_tic_tac_toe_bdd_0nodes.tex <==
485.0        0.672 % 16
2077.6       1.0588 % 17
10292.8      1.2533 % 18
59283.9      1.5000 % 19
332937.3     1.7237 % 20
1767478.8    1.9474 % 21
8555218.2    2.1579 % 22
36573231.9   2.3553 % 23
132606027.39 2.5132 % 24


==> data/ppr_unweighted_tic_tac_toe_bdd_1level.tex <==
485.0        13.194 % 16
2077.6       14.103 % 17
10292.8      14.000 % 18
59283.9      13.987 % 19
332937.3     14.066 % 20
1767478.8    14.158 % 21
8555218.2    14.263 % 22
36573231.9   14.316 % 23
132606027.39 14.408 % 24


==> data/ppr_unweighted_tic_tac_toe_bdd_2level.tex <==
485.0        16.597 % 16
2077.6       16.324 % 17
10292.8      16.040 % 18
59283.9      15.934 % 19
332937.3     16.118 % 20
1767478.8    16.316 % 21
8555218.2    16.526 % 22
36573231.9   16.763 % 23
132606027.39 16.987 % 24


==> data/ppr_unweighted_tic_tac_toe_zdd_0nodes.tex <==
246.8       0.134 % 16
1153.7      0.1471 % 17
6138.7      0.1467 % 18
39596.8     0.1447 % 19
245775.4    0.1579 % 20
1408529.2   0.1711 % 21
7207145.8   0.1842 % 22
32002420.4  0.1842 % 23
118781618.5 0.1974 % 24


==> data/ppr_unweighted_tic_tac_toe_zdd_1level.tex <==
246.8       6.269 % 16
1153.7      6.353 % 17
6138.7      6.600 % 18
39596.8     6.724 % 19
245775.4    7.053 % 20
1408529.2   7.421 % 21
7207145.8   7.763 % 22
32002420.4  8.079 % 23
118781618.5 8.342 % 24


==> data/ppr_unweighted_tic_tac_toe_zdd_2level.tex <==
246.8       8.791 % 16
1153.7      8.603 % 17
6138.7      8.680 % 18
39596.8     8.724 % 19
245775.4    9.092 % 20
1408529.2   9.526 % 21
7207145.8   9.921 % 22
32002420.4  10.316 % 23
118781618.5 10.658 % 24


==> data/ppr_weighted_knights_tour_0nodes.tex <==
32       0.3685 % 5  (open)
176      0.1666 % 6  (open)
276      0.0749 % 7  (open)
586      0.0472 % 8  (open)
1103     0.0281 % 9  (open)
586787   0.0152 % 10 (open)
1669329  0.0091 % 11 (open)
63056257 0.0059 % 12 (open)
34       0.2197 % 6  (closed)
76       0.1119 % 7  (closed)
390      0.0524 % 8  (closed)
17824    0.0292 % 9  (closed)
605      0.0117 % 10 (closed)
139833   0.0096 % 11 (closed)
1219497  0.0056 % 12 (closed)
39304233 0.0042 % 13 (closed)
4322     0.0015 % 14 (closed)


==> data/ppr_weighted_knights_tour_1level.tex <==
32       6.5395 % 5  (open)
176      1.8061 % 6  (open)
276      1.3382 % 7  (open)
586      1.2761 % 8  (open)
1103     1.1229 % 9  (open)
586787   0.9296 % 10 (open)
1669329  0.7255 % 11 (open)
63056257 0.5916 % 12 (open)
34       1.7316 % 6  (closed)
76       1.2115 % 7  (closed)
390      0.9456 % 8  (closed)
17824    0.8870 % 9  (closed)
605      0.2434 % 10 (closed)
139833   0.7816 % 11 (closed)
1219497  0.6046 % 12 (closed)
39304233 0.5056 % 13 (closed)
4322     0.0945 % 14 (closed)


==> data/ppr_weighted_knights_tour_2level.tex <==
32       6.5395 % 5  (open)
176      2.5303 % 6  (open)
276      1.9207 % 7  (open)
586      1.8588 % 8  (open)
1103     1.6564 % 9  (open)
586787   1.3684 % 10 (open)
1669329  1.0756 % 11 (open)
63056257 0.8822 % 12 (open)
34       1.9629 % 6  (closed)
76       1.6187 % 7  (closed)
390      1.3504 % 8  (closed)
17824    1.2808 % 9  (closed)
605      0.3531 % 10 (closed)
139833   1.1420 % 11 (closed)
1219497  0.8908 % 12 (closed)
39304233 0.7448 % 13 (closed)
4322     0.1402 % 14 (closed)


==> data/ppr_weighted_picotrav_0nodes.tex <==
794       0.0721    % adder     (depth)
1114064   0.0010    % sin       (depth)
98        5.1331    % cavlc     (depth)
15        9.9680    % ctrl      (depth)
8         5.3423    % dec       (depth)
261       9.1097    % i2c       (depth)
153       7.5220    % int2float (depth)
128       0.4970    % priority  (depth)
126       2.2432    % router    (depth)
360039226 0.0000001 % voter     (depth)
387       0.0495    % adder     (size)
1111220   0.0008    % sin       (size)
2780488   0.0224    % arbiter   (size)
261       9.8207    % i2c       (size)
153       9.8207    % int2float (size)
216       0.5215    % priority  (size)
126       2.3969    % router    (size)
360039226 0.0000003 % voter     (size)



==> data/ppr_weighted_picotrav_1level.tex <==
794       10.6446   % adder     (depth)
1114064   0.0010    % sin       (depth)
98        10.7063   % cavlc     (depth)
15        25.8396   % ctrl      (depth)
8         29.1457   % dec       (depth)
261       18.3266   % i2c       (depth)
153       14.4674   % int2float (depth)
128       18.9885   % priority  (depth)
126       14.5994   % router    (depth)
360039226 0.0003    % voter     (depth)
387       25.7552   % adder     (size)
1111220   0.0009    % sin       (size)
2780488   0.0341    % arbiter   (size)
261       20.1454   % i2c       (size)
153       48.9692   % int2float (size)
216       17.2680   % priority  (size)
126       15.7032   % router    (size)
360039226 0.0004282 % voter     (size)



==> data/ppr_weighted_picotrav_2level.tex <==
794       14.2149   % adder     (depth)
1114064   0.0011    % sin       (depth)
98        13.6517   % cavlc     (depth)
15        29.2225   % ctrl      (depth)
8         29.1457   % dec       (depth)
261       23.4461   % i2c       (depth)
153       20.6350   % int2float (depth)
128       19.1741   % priority  (depth)
126       17.6959   % router    (depth)
360039226 0.0006    % voter     (depth)
387       37.9397   % adder     (size)
1111220   0.0009    % sin       (size)
2780488   0.0402    % arbiter   (size)
261       25.9930   % i2c       (size)
153       64.2206   % int2float (size)
216       18.5860   % priority  (size)
126       19.6361   % router    (size)
360039226 0.0006    % voter     (size)



==> data/ppr_weighted_queens_bdd_0nodes.tex <==
109       0.8518 % 4
368       0.2746 % 5
1143      0.0956 % 6
3270      0.0226 % 7
10705     0.0058 % 8
44110     0.0013 % 9
212596    0.0003 % 10
1027599   0.0001 % 11
4938578   0.0000 % 12
26724679  0.0000 % 13
153283605 0.0000 % 14
868017400 0.0000 % 15


==> data/ppr_weighted_queens_bdd_1level.tex <==
109       9.3502 % 4
368       5.3619 % 5
1143      2.6867 % 6
3270      1.0771 % 7
10705     0.3991 % 8
44110     0.1353 % 9
212596    0.0460 % 10
1027599   0.0161 % 11
4938578   0.0061 % 12
26724679  0.0026 % 13
153283605 0.0012 % 14
868017400 0.0006 % 15


==> data/ppr_weighted_queens_bdd_2level.tex <==
109       11.5800 % 4
368       7.5493 % 5
1143      3.9956 % 6
3270      1.7662 % 7
10705     0.6705 % 8
44110     0.2320 % 9
212596    0.0763 % 10
1027599   0.0266 % 11
4938578   0.0100 % 12
26724679  0.0042 % 13
153283605 0.0019 % 14
868017400 0.0009 % 15


==> data/ppr_weighted_queens_zdd_0nodes.tex <==
85        3.9695 % 4
367       1.0567 % 5
1303      0.3208 % 6
3994      0.0822 % 7
11297     0.0225 % 8
30142     0.0059 % 9
77427     0.0017 % 10
192974    0.0005 % 11
779246    0.0002 % 12
3778062   0.0001 % 13
19483072  0.0000 % 14
110468521 0.0000 % 15
634184585 0.0000 % 16


==> data/ppr_weighted_queens_zdd_1level.tex <==
85        12.3652 % 4 
367       5.6618 % 5
1303      2.4916 % 6
3994      0.9588 % 7
11297     0.3420 % 8
30142     0.1174 % 9
77427     0.0433 % 10
192974    0.0170 % 11
779246    0.0072 % 12
3778062   0.0033 % 13
19483072  0.0016 % 14
110468521 0.0008 % 15
634184585 0.0004 % 16


==> data/ppr_weighted_queens_zdd_2level.tex <==
85        19.9305 % 4 
367       9.5247 % 5
1303      4.0356 % 6
3994      1.5038 % 7
11297     0.5248 % 8
30142     0.1814 % 9
77427     0.0664 % 10
192974    0.0258 % 11
779246    0.0109 % 12
3778062   0.0050 % 13
19483072  0.0024 % 14
110468521 0.0012 % 15
634184585 0.0006 % 16


==> data/ppr_weighted_tic_tac_toe_bdd_0nodes.tex <==
1182      0.6455 % 16
9069      1.0544 % 17
54979     1.2344 % 18
337580    1.4113 % 19
1868144   1.6299 % 20
9624972   1.9236 % 21
46630372  2.2556 % 22
214204811 2.5917 % 23
801053452 2.9176 % 24


==> data/ppr_weighted_tic_tac_toe_bdd_1level.tex <==
1182      12.7349 % 16
9069      14.9335 % 17
54979     14.8364 % 18
337580    15.0927 % 19
1868144   15.1181 % 20
9624972   14.9878 % 21
46630372  14.7023 % 22
214204811 14.3704 % 23
801053452 14.1234 % 24


==> data/ppr_weighted_tic_tac_toe_bdd_2level.tex <==
1182      16.3255 % 16
9069      16.7450 % 17
54979     15.7597 % 18
337580    15.5845 % 19
1868144   15.5496 % 20
9624972   15.3243 % 21
46630372  15.0082 % 22
214204811 14.7570 % 23
801053452 14.5999 % 24


==> data/ppr_weighted_tic_tac_toe_zdd_0nodes.tex <==
726       0.1220 % 16
4318      0.1323 % 17
31053     0.1298 % 18
218170    0.1314 % 19
1462967   0.1371 % 20
8040730   0.1472 % 21
40047272  0.1584 % 22
191772820 0.1697 % 23
737600983 0.1811 % 24


==> data/ppr_weighted_tic_tac_toe_zdd_1level.tex <==
726       4.8435 % 16
4318      6.1777 % 17
31053     6.1008 % 18
218170    6.0690 % 19
1462967   6.2603 % 20
8040730   6.5337 % 21
40047272  6.7788 % 22
191772820 7.0026 % 23
737600983 7.2195 % 24


==> data/ppr_weighted_tic_tac_toe_zdd_2level.tex <==
726       6.2580 % 16
4318      8.1957 % 17
31053     7.9312 % 18
218170    7.8540 % 19
1462967   7.8814 % 20
8040730   7.9974 % 21
40047272  8.1325 % 22
191772820 8.2502 % 23
737600983 8.4363 % 24


==> data/time_knights_tour_closed_0nodes__128MiB.tex <==
1        0 % 1x1
1079     12 % 3x3
3223     32 % 4x3
10391    72 % 4x4
31132    188 % 5x4
38601    77 % 5x5
890895   3721 % 6x5
15189531 85416 % 6x6


==> data/time_knights_tour_closed_1level__128MiB.tex <==
1        0 % 1x1
1079     13 % 3x3
3223     31 % 4x3
10391    71 % 4x4
31132    159 % 5x4
38601    73 % 5x5
890895   3210 % 6x5
15189531 83318 % 6x6


==> data/time_knights_tour_closed_2level__128MiB.tex <==
1        0 % 1x1
1079     12 % 3x3
3223     32 % 4x3
10391    73 % 4x4
31132    158 % 5x4
38601    75 % 5x5
890895   3141 % 6x5
15189531 84058 % 6x6


==> data/time_knights_tour_open_0nodes__128MiB.tex <==
1        0      % 1x1
1        1      % 2x1
1        4      % 2x2
140      11     % 3x2
1459     35     % 3x3
6696     92     % 4x3
57836    364    % 4x4
327987   1429   % 5x4
3461700  14560  % 5x5
22968247 148999 % 6x5


==> data/time_knights_tour_open_1level__128MiB.tex <==
1        0      % 1x1
1        1      % 2x1
1        4      % 2x2
140      10     % 3x2
1459     35     % 3x3
6696     91     % 4x3
57836    310    % 4x4
327987   1255   % 5x4
3461700  14199  % 5x5
22968247 144668 % 6x5


==> data/time_knights_tour_open_2level__128MiB.tex <==
1        0      % 1x1
1        1      % 2x1
1        3      % 2x2
140      11     % 3x2
1459     35     % 3x3
6696     92     % 4x3
57836    315    % 4x4
327987   1243   % 5x4
3461700  14334  % 5x5
22968247 146104 % 6x5


==> data/time_queens_bdd_0nodes__128MiB.tex <==
642       17     % 4
2578      29     % 5
8341      46     % 6
29240     84     % 7
96242     143    % 8
339457    289    % 9
1249096   776    % 10
5115514   2943   % 11
23326222  15288  % 12
117065779 102691 % 13
637044763 857935 % 14


==> data/time_queens_bdd_1level__128MiB.tex <==
642       16     % 4
2578      28     % 5
8341      44     % 6
29240     69     % 7
96242     120    % 8
339457    282    % 9
1249096   760    % 10
5115514   2832   % 11
23326222  14251  % 12
117065779 92955  % 13
637044763 851355 % 14


==> data/time_queens_bdd_2level__128MiB.tex <==
642       16     % 4
2578      29     % 5
8341      46     % 6
29240     73     % 7
96242     122    % 8
339457    285    % 9
1249096   790    % 10
5115514   2967   % 11
23326222  14961  % 12
117065779 97854  % 13
637044763 891046 % 14


==> data/time_queens_zdd_0nodes__128MiB.tex <==
389       17     % 4
1928      28     % 5
7491      44     % 6
26187     80     % 7
83570     140    % 8
257038    279    % 9
774405    718    % 10
2387342   2371   % 11
7840149   11253  % 12
28591268  73227  % 13
119917860 535896 % 14


==> data/time_queens_zdd_1level__128MiB.tex <==
389       16     % 4
1928      27     % 5
7491      43     % 6
26187     68     % 7
83570     117    % 8
257038    255    % 9
774405    654    % 10
2387342   2181   % 11
7840149   10828  % 12
28591268  71029  % 13
119917860 529869 % 14


==> data/time_queens_zdd_2level__128MiB.tex <==
389       16     % 4
1928      27     % 5
7491      44     % 6
26187     70     % 7
83570     118    % 8
257038    266    % 9
774405    674    % 10
2387342   2251   % 11
7840149   11115  % 12
28591268  71846  % 13
119917860 536528 % 14


==> data/time_ratio_knights_tour_closed_1level__128MiB.tex <==
34      8.33 % 3x3
76      -3.13 % 4x3
390     -1.39 % 4x4
17824   -15.43 % 5x4
605     -5.19 % 5x5
139833  -13.73 % 6x5
1219497 -2.46 % 6x6


==> data/time_ratio_knights_tour_closed_1level__4GiB.tex <==
34      -7.69 % 3x3
76      2.94 % 4x3
390     2.70 % 4x4
17824   -0.63 % 5x4
605     0.00 % 5x5
139833  -29.73 % 6x5
1219497 -18.47 % 6x6


==> data/time_ratio_knights_tour_closed_2level__128MiB.tex <==
34      0.00 % 3x3
76      0.00 % 4x3
390     1.39 % 4x4
17824   -15.96 % 5x4
605     -2.60 % 5x5
139833  -15.59 % 6x5
1219497 -1.59 % 6x6


==> data/time_ratio_knights_tour_closed_2level__4GiB.tex <==
34      -7.69 % 3x3
76      0.00 % 4x3
390     4.05 % 4x4
17824   2.52 % 5x4
605     2.67 % 5x5
139833  -28.89 % 6x5
1219497 -17.71 % 6x6


==> data/time_ratio_knights_tour_open_1level__128MiB.tex <==
32       -9.09 % 3x2
176       0.00 % 3x3
276      -1.09 % 4x3
586     -14.84 % 4x4
1103    -12.18 % 5x4
586787   -2.48 % 5x5
1669329  -2.91 % 6x5


==> data/time_ratio_knights_tour_open_1level__4GiB.tex <==
32      -9.09 % 3x2
176     2.70 % 3x3
276     -1.08 % 4x3
586     -0.64 % 4x4
1103    -12.15 % 5x4
586787  -18.34 % 5x5
1669329 -15.13 % 6x5


==> data/time_ratio_knights_tour_open_2level__128MiB.tex <==
32        0.00 % 3x2
176       0.00 % 3x3
276       0.00 % 4x3
586     -13.46 % 4x4
1103    -13.02 % 5x4
586787   -1.55 % 5x5
1669329  -1.94 % 6x5


==> data/time_ratio_knights_tour_open_2level__4GiB.tex <==
32      -9.09 % 3x2
176     0.00 % 3x3
276     0.00 % 4x3
586     0.64 % 4x4
1103    -10.22 % 5x4
586787  -17.22 % 5x5
1669329 -15.40 % 6x5


==> data/time_ratio_picotrav_1level__128MiB.tex <==
794        -1.53 % adder     (depth)
98         0.41 % cavlc     (depth)
15         -0.38 % ctrl      (depth)
8          0.53 % dec       (depth)
261        -1.71 % i2c       (depth)
153        -5.73 % int2float (depth)
128        -2.49 % priority  (depth)
126        -1.32 % router    (depth)
387        -2.75 % adder     (size)
1111220    -0.06 % sin       (size)
2780488    -1.39 % arbiter   (size)
15         -1.58 % cavlc     (size)
8          -0.38 % ctrl      (size)
261        -0.53 % dec       (size)
261        2.57 % i2c       (size)
153        0.14 % int2float (size)
216        -7.00 % priority  (size)
126        -0.34 % router    (size)


==> data/time_ratio_picotrav_1level__4GiB.tex <==
794        -0.52 % adder     (depth)
98         -3.84 % cavlc     (depth)
15         -0.83 % ctrl      (depth)
8          -1.89 % dec       (depth)
261        -2.36 % i2c       (depth)
153        -2.72 % int2float (depth)
128        -2.43 % priority  (depth)
126        -3.06 % router    (depth)
387        0.89 % adder     (size)
1111220    0.65 % sin       (size)
2780488    -1.95 % arbiter   (size)
15         2.46 % cavlc     (size)
8          -5.44 % ctrl      (size)
261        -3.86 % dec       (size)
261        -3.05 % i2c       (size)
153        -6.48 % int2float (size)
216        -3.67 % priority  (size)
126        -2.42 % router    (size)


==> data/time_ratio_picotrav_2level__128MiB.tex <==
794        0.33 % adder     (depth)
98         -0.94 % cavlc     (depth)
15         5.95 % ctrl      (depth)
8          -0.36 % dec       (depth)
261        -1.99 % i2c       (depth)
153        -2.15 % int2float (depth)
128        -0.88 % priority  (depth)
126        -0.33 % router    (depth)
387        0.21 % adder     (size)
1111220    2.44 % sin       (size)
2780488    0.73 % arbiter   (size)
15         -0.04 % cavlc     (size)
8          3.06 % ctrl      (size)
261        5.59 % dec       (size)
261        -4.01 % i2c       (size)
153        -0.28 % int2float (size)
216        -6.16 % priority  (size)
126        -1.20 % router    (size)


==> data/time_ratio_picotrav_2level__4GiB.tex <==
794        -0.09 % adder     (depth)
98         -0.82 % cavlc     (depth)
15         1.78 % ctrl      (depth)
8          1.05 % dec       (depth)
261        0.30 % i2c       (depth)
153        -1.34 % int2float (depth)
128        3.56 % priority  (depth)
126        2.10 % router    (depth)
387        2.07 % adder     (size)
1111220    4.68 % sin       (size)
2780488    -1.06 % arbiter   (size)
15         -3.86 % cavlc     (size)
8          -2.54 % ctrl      (size)
261        -3.24 % dec       (size)
261        -1.38 % i2c       (size)
153        -2.82 % int2float (size)
216        -1.33 % priority  (size)
126        -1.90 % router    (size)


==> data/time_ratio_queens_bdd_1level__128MiB.tex <==
109       -5.88  % 4
368       -3.45  % 5
1143      -4.35  % 6
3270     -17.86  % 7
10705    -16.08  % 8
44110     -2.42  % 9
212596    -2.06  % 10
1027599   -3.77  % 11
4938578   -6.78  % 12
26724679  -9.48  % 13
153283605 -0.77  % 14


==> data/time_ratio_queens_bdd_1level__4GiB.tex <==
109       -5.88  % 4
368       0.00   % 5
1143      -2.13  % 6
3270      1.41   % 7
10705     -30.77 % 8
44110     -25.51 % 9
212596    -10.46 % 10
1027599   -2.58  % 11
4938578   -3.61  % 12
26724679  -1.53  % 13
153283605 -3.49  % 14


==> data/time_ratio_queens_bdd_2level__128MiB.tex <==
109       -5.88  % 4
368        0.00 % 5
1143       0.00 % 6
3270     -13.10 % 7
10705    -14.69 % 8
44110     -1.38 % 9
212596     1.80 % 10
1027599    0.82 % 11
4938578   -2.14 % 12
26724679  -4.71 % 13
153283605  3.86 % 14


==> data/time_ratio_queens_bdd_2level__4GiB.tex <==
109         5.88 % 4
368         3.45 % 5
1143        2.13 % 6
3270        5.63 % 7
10705     -27.22 % 8
44110     -23.46 % 9
212596    -12.37 % 10
1027599     1.67 % 11
4938578     0.59 % 12
26724679    4.30 % 13
153283605   1.61 % 14


==> data/time_ratio_queens_zdd_1level__128MiB.tex <==
85       -5.88  % 4
367      -3.57  % 5
1303     -2.27  % 6
3994     -15.00 % 7
11297    -16.43 % 8
30142    -8.60  % 9
77427    -8.91  % 10
192974   -8.01  % 11
779246   -3.78  % 12
3778062  -3.00  % 13
19483072 -1.12  % 14


==> data/time_ratio_queens_zdd_1level__4GiB.tex <==
85       -11.11  % 4
367      0.00  % 5
1303     -8.70  % 6
3994     1.45 % 7
11297    0.86 % 8
30142    -23.36  % 9
77427    -10.29  % 10
192974   -3.88  % 11
779246   -1.01  % 12
3778062  -1.91  % 13
19483072 -1.12  % 14


==> data/time_ratio_queens_zdd_2level__128MiB.tex <==
85       -5.88  % 4
367      -3.57  % 5
1303      0.00  % 6
3994     -12.50 % 7
11297    -15.71 % 8
30142    -4.66  % 9
77427    -6.13  % 10
192974   -5.06  % 11
779246   -1.23  % 12
3778062  -1.89  % 13
19483072  0.12  % 14


==> data/time_ratio_queens_zdd_2level__4GiB.tex <==
85       -11.11  % 4
367      0.00  % 5
1303     -2.17  % 6
3994     2.90 % 7
11297    5.17 % 8
30142    -20.07  % 9
77427    -10.71  % 10
192974   -0.98  % 11
779246   1.58  % 12
3778062  0.85  % 13
19483072 0.92  % 14


==> data/time_ratio_tic_tac_toe_bdd_1level__128MiB.tex <==
1182     -0.54 % 16
9069     0.80 % 17
54979    -1.47 % 18
337580   -3.51 % 19
1868144  -13.01 % 20
9624972  -8.20 % 21
46630372 -0.48 % 22


==> data/time_ratio_tic_tac_toe_bdd_1level__4GiB.tex <==
1182     0.53 % 16
9069     -0.79 % 17
54979    -1.93 % 18
337580   0.60 % 19
1868144  -1.94 % 20
9624972  -4.91 % 21
46630372 -5.27 % 22


==> data/time_ratio_tic_tac_toe_bdd_2level__128MiB.tex <==
1182     -2.70 % 16
9069     3.59 % 17
54979    5.55 % 18
337580   1.84 % 19
1868144  -9.53 % 20
9624972  -3.84 % 21
46630372 4.24 % 22


==> data/time_ratio_tic_tac_toe_bdd_2level__4GiB.tex <==
1182     -1.60 % 16
9069     2.76 % 17
54979    4.66 % 18
337580   6.76 % 19
1868144  4.79 % 20
9624972  1.84 % 21
46630372 0.33 % 22


==> data/time_ratio_tic_tac_toe_zdd_1level__128MiB.tex <==
726      0.00 % 16
4318     -2.70 % 17
31053    -14.78 % 18
218170   -10.28 % 19
1462967  -4.45 % 20
8040730  -2.40 % 21
40047272 -0.09 % 22

==> data/time_ratio_tic_tac_toe_zdd_1level__4GiB.tex <==
726       5.23 % 16
4318     -1.14 % 17
31053     1.85 % 18
218170   -4.87 % 19
1462967 -10.77 % 20
8040730  -7.51 % 21
40047272 -2.35 % 22

==> data/time_ratio_tic_tac_toe_zdd_2level__128MiB.tex <==
726      -0.59 % 16
4318     -0.77 % 17
31053    -12.85 % 18
218170   -6.96 % 19
1462967  -1.74 % 20
8040730  0.18 % 21
40047272 2.82 % 22

==> data/time_ratio_tic_tac_toe_zdd_2level__4GiB.tex <==
726       1.74 % 16
4318     -1.14 % 17
31053     6.34 % 18
218170   -2.05 % 19
1462967  -6.15 % 20
8040730  -5.29 % 21
40047272  1.52 % 22

==> data/time_tic_tac_toe_bdd_0nodes__128MiB.tex <==
32495     185    % 16
141279    251    % 17
771958    613    % 18
4505573   2452   % 19
25303238  16390  % 20
134328389 111296 % 21
650196580 880244 % 22


==> data/time_tic_tac_toe_bdd_1level__128MiB.tex <==
32495     184    % 16
141279    253    % 17
771958    604    % 18
4505573   2366   % 19
25303238  14258  % 20
134328389 102168 % 21
650196580 876054 % 22


==> data/time_tic_tac_toe_bdd_2level__128MiB.tex <==
32495     180    % 16
141279    260    % 17
771958    647    % 18
4505573   2497   % 19
25303238  14828  % 20
134328389 107019 % 21
650196580 917605 % 22


==> data/time_tic_tac_toe_zdd_0nodes__128MiB.tex <==
17320     170     % 16
79270     259     % 17
461240    778     % 18
3009354   3335    % 19
18679829  24312   % 20
107049143 187928  % 21
547744025 1399211 % 22


==> data/time_tic_tac_toe_zdd_1level__128MiB.tex <==
17320     170     % 16
79270     252     % 17
461240    663     % 18
3009354   2992    % 19
18679829  23231   % 20
107049143 183420  % 21
547744025 1397947 % 22


==> data/time_tic_tac_toe_zdd_2level__128MiB.tex <==
17320     169     % 16
79270     257     % 17
461240    678     % 18
3009354   3103    % 19
18679829  23889   % 20
107049143 188271  % 21
547744025 1438702 % 22


==> figure/i-level_cut_definition_and_examples.tex <==
\begin{figure}[t]
  \centering

  \subfloat[Definition of an $i$-level cut.]{
    \label{fig:i-level_cut_definition}

    \centering
    \begin{tikzpicture}[scale=0.9]
      \input{tikz/i-level_cut_definition.tex}
    \end{tikzpicture}
  }
  \quad
  \subfloat[Example of cuts in a BDD.]{
    \label{fig:i-level_cut_examples}

    \centering
    \begin{tikzpicture}
      \input{tikz/i-level_cut_examples.tex}
    \end{tikzpicture}
  }

  \caption{Visualization of $i$-level (purple), $1$-level (cyan) and
    $2$-level (orange) cuts.}
\end{figure}

==> table/bdd_operations.tex <==
\if\arxiv1
\begin{table}[ht!]
\else
\begin{table}[t]
\fi
  \centering
  \small

  \caption{BDD operations and their time complexity in the \Adiar\ BDD package.
    Here $N_f$ is the size of the BDD representing $f$ and $\sort(N) \triangleq
    N \log N$.}
  \label{tab:bdd_operations}

  \begin{tabular}{l l | c}
    \multicolumn{2}{c|}{Algorithm} & Time Complexity
    \\ \hline \hline
    \multicolumn{3}{c}{BDD Manipulation}
    \\ \hline
    Apply             & $f \odot g$
                      & $O(\sort(N_f N_g))$
    \\
%    Composition       & $f[g/x_i]$
%                      & $O(\sort(N_f^2 N_g))$
%    \\
    If-Then-Else      & $(f \land g) \vee (\neg f \land h)$
                      & $O(\sort(N_f N_g N_h)$
    \\
%    Negation          & $\neg f$
%                      & $O(1)$
%    \\
    Restrict          & $f[b/x_i]$
                      & $O(\sort(N_f))$
    \\
    Quantification    & $\exists/\forall\ b : f[b/x_i]$
                      & $O(\sort(N_f^2))$
    \\ \hline
    \multicolumn{3}{c}{Other}
    \\ \hline
    Count SAT         & $\abs{\{ x \in \{ 0,1 \}^n \mid f(x) \equiv \top \}}$
                      & $O(\sort(N_f))$
    \\
    Isomorphism       & $f \equiv g$
                      & $O(\sort(\min(N_f, N_g)))$
  \end{tabular}
\end{table}


==> table/picotrav_precision.tex <==
\if\arxiv1
\begin{table}[ht]
\else
\begin{table}[t]
  \fi
  \centering

  \caption{Ratio between the predicted and the actual maximum size of the binary
    Equality Checking operation's priority queue.}
  \label{tab:picotrav_precision}

  \subfloat[Ratio for single output of an EPFL Circuit. These were all optimised
  for depth.]{
    \begin{tabular}{r || c || c|c|c}
      & PQ Size & \ \#nodes \ & \ $1$-level \ & \ $2$-level
      \\ \hline
      \texttt{int2float}
      & 4       & 40\%        & 80\%          & 80\%
      \\
      \texttt{router}
      & 27      & 21\%        & 69\%          & 93\%
      \\
      \texttt{voter}
      & 1000    & 0.4\%       & 67\%          & 100\%
    \end{tabular}
  }

  \subfloat[Geometric Mean]{
    \begin{tabular}{r || c|c|c}
      & \ \#nodes \ & \ $1$-level \ & \ $2$-level
      \\ \hline
      Unweighted Avg.
      &
        2.1\%         & 69.2\%        & 86.3\%
      \\
      Weighted Avg.
      &
        0.1\%         & 76.5\%        & 77.4\%
    \end{tabular}
  }
\end{table}
